FlashCheck: Exploration of Efficient Evidence Retrieval for Fast Fact-Checking

The advances in digital tools have led to the rampant spread of misinformation. While fact-checking aims to combat this, manual fact-checking is cumbersome and not scalable. It is essential for automated fact-checking to be efficient for aiding in combating misinformation in real-time and at the source. Fact-checking pipelines primarily comprise a knowledge retrieval component which extracts relevant knowledge to fact-check a claim from large knowledge sources like Wikipedia and a verification component. The existing works primarily focus on the fact-verification part rather than evidence retrieval from large data collections, which often face scalability issues for practical applications such as live fact-checking. In this study, we address this gap by exploring various methods for indexing a succinct set of factual statements from large collections like Wikipedia to enhance the retrieval phase of the fact-checking pipeline. We also explore the impact of vector quantization to further improve the efficiency of pipelines that employ dense retrieval approaches for first-stage retrieval. We study the efficiency and effectiveness of the approaches on fact-checking datasets such as HoVer and WiCE, leveraging Wikipedia as the knowledge source. We also evaluate the real-world utility of the efficient retrieval approaches by fact-checking 2024 presidential debate and also open source the collection of claims with corresponding labels identified in the debate. Through a combination of indexed facts together with Dense retrieval and Index compression, we achieve up to a 10.0x speedup on CPUs and more than a 20.0x speedup on GPUs compared to the classical fact-checking pipelines over large collections.

==> 01-intro-AA.tex <==
\section{Introduction (2 pages)}
\label{sec:intro}
\input{tables/table-intro-anecdotal}


In Information Retrieval (IR), the discrepancy between user queries and documents, termed ``vocabulary mismatch'' is a central problem. 
User queries, often in keyword form, might be ambiguous and unclear, making it challenging to discern user intentions, which in turn influences retrieval accuracy. 
For instance, the query \texttt{define sri} could refer to ``sanskrit word sri'' or ``\textbf{S}ocially \textbf{R}esponsible \textbf{I}nvestment''.
Consequently, to disambiguate the users' information need, classical approaches like pseudo-relevance feedback mechanism \cite{lv2009comparative,ir_query_exp}, KNN-search \cite{grbovic2015context,zamani:2017:relevance-based-word-embedding,he2016learning} expand the original query with keywords from top-ranked results to the original query. 
However, all the above approaches are term-based approaches that improve retrieval but not document ranking and lack interpretability.  \note{Avishek}{Previous sentence is confusing.}
Going beyond keywords, researchers have explored the possibility of natural language generation for clarifying queries~\cite{rao2018learning,zerveas2020brown,doc2query}.
Recently, LLMs have shown of large language models or LLMs~\cite{gpt3_prompting,gpt3incontext}, recent approaches have started to investigate the utility of LLMs to aid in enriching query and document representations~\cite{wang2023query2doc,gospodinov2023doc2query}. 
However, there are two major limitations to using LLMs for the task of query re-writing -- misaligned intent ?? and high inference costs and latency.


\mpara{The problem of misaligned intents.}
When using LLM-based query expansions, the expanded query results in choosing one aspect among the many possible aspects as query might have.
This entails in a problem that the chosen intent by the expansion might not align with the ground-truth intent due to topic drift or the issue of hallucination when generating long context for a given query.
Specifically, such intent non-alignment results in the case of forced match of an erroneously expanded query and a document. For instance, in Table~\ref{tab:intro_anecdotal}, we observe that for the query \texttt{define sri}, \qd{} drifts away from the intent and generates a query related to \textit{Stanford Research Institute }instead of denoting the Sanskrit word.  

\mpara{The problem of efficient inference.}
Secondly, a serious limitation (as acknowledged  in~\cite{wang2023query2doc}) is the computational overhead from both the retrieval and re-ranking phases.
The query expansions use the expensive tokenwise auto-regressive decoding during inference. Therefore, to stay within sub-second ranking requirements without using prohibitively expensive compute the choice of a LLM during query processing should be avoided.


\mpara{Context Aware Generative Query Enrichment.}
We make two simple yet important design decisions to overcome the problem of misalignment and efficiency.
Firstly, we generate query rewrites using LLMs by additionally providing the relevant document as context during training. 
Secondly, and unlike existing works, we fully avoid any query rewriting using LLMs \textbf{during inference}. 

Methodologically, we propose an LLM-based context-aware query enrichment framework \car{}, that replaces the traditional query rewriter with a LLM for rewriting ambiguous queries. 
At \textbf{inference time}, the ranker fine-tuned on rewritten queries, is equipped with knowledge of query disambiguation mechanism and improves the document ranking performance for subsequent ambiguous queries without the rewriter component. The proposed framework can be used with any off-the-shelf ranker. 
From Table \ref{tab:intro_anecdotal} we observe that the proposed context-aware query reformulation approach \car{}, can generate concise rewrites that reflect the intent when compared to \qd{} and other approaches. 


\mpara{The need for identification of ambiguous queries}: Our primary goal is to ameliorate the document ranking performance for ambiguous queries without compromising performance on other queries. The ranker fine-tuned only on rewritten ambiguous queries specializes in improving the document ranking performance for similar ambiguous queries. While the ranker fine-tuned on all queries (\textit{base ranker}) can be employed for well-formed queries. Hence, automated identification of ambiguous queries aid in routing them to the \textit{specialized ranker} and rest of the queries to the base ranker. Inspired by BERT-QPP \cite{bert_qpp}, we propose to use a post-retrieval neural Query Performance Predictor (QPP) fine-tuned to predict performance of a query based on initial document set retrieved using sparse methods like BM25. During inference, the QPP model is used to categorize a query as ambiguous based on the performance score predicted and is used to weigh the relevance scores from both ranking models.

We perform extensive experiments using LLMs of different parameter scales and demonstrate that the proposed approach results in better ranking performance. 
Specifically, we find that fine-tuning a ranker using re-written queries offers a significant improvement of up to \textbf{33\%} on the passage ranking task and up to \textbf{23\%} on the document ranking task when compared to the baseline performance of using original queries.


\noindent In summary, here is a list of our \textbf{contributions}: 
\begin{enumerate}
    \item We propose the use of existing techniques aimed at efficiently identifying relevant text spans from large corpora pertaining to the claims being fact-checked, enabling more targeted retrieval and verification processes.
    
    \item We show the methods for indexing supporting facts optimizes retrieval efficiency by reducing computational overhead and accelerating the retrieval process.
    
    \item We show a comprehensive evaluation of various retrieval approaches, mainly showing the difference of effectiveness and efficiency in indexing supporting facts versus indexing the entire data corpus. 
\end{enumerate}

==> 03-method_new.tex <==
\begin{figure*}[hbt!]
    \centering
    % \includegraphics [width=0.57\textwidth]{figs/ictir_figure.pdf}
    \includegraphics [width=1.05\textwidth]{figs/ecir_2024_cagqer.pdf}
    \caption{Overview of the proposed \car{} framework and inference workflow}
    \label{system}
\end{figure*}
\section{Method}

%\todo {Rewrite this Section 3 so as to describe our approach and include reference to subsections.}
%In this section, we describe the proposed Context Aware Query Enrichment Ranking framework for ambiguous query reformulation. Figure \ref{system} shows the working of the proposed framework during the training and inference stages. During training, we employ a context-aware prompting of a LLM (\car{}) (Section \ref{rewriter:method}) to get query rewrites and use them to fine-tune a ranker specialized for ambiguous queries. During inference, the ambiguous queries are identified based on the query performance scores obtained using a fine-tuned query performance predictor model. Then the specialized ranker and base ranker are directly employed to rank documents for new queries without rewriting them, as shown in Figure \ref{system}. The relevance scores from both the approaches are combined using rank fusion, yielding the final ranked list.

%In this section, we describe the proposed Context Aware Query Enrichment Ranking framework for ambiguous query reformulation. Figure \ref{system} shows the proposed framework during the training and inference stages. During training, we utilize LLMs(CAQE)(Section \ref{rewriter:method}), to generate alternative query formulations. These rewritten queries serve as training data for our specialised ranker for ambiguous queries(SR). During inference we first get query performance using a trained QPP(Section \ref{method:qpp}) model and then use the predictor score along with  rank fusion to get the final ranking.

In this section, we describe our proposed ranking framework as shown in Figure \ref{system}. It consists of two stages, In first stage, we enrich hard queries using LLMs (\car{})(Section \ref{rewriter:method}). We then train two models, one where enriched queries serve as training data for a specialized ranker for hard queries ($SR$) and the other using the original queries ($BR$)(Section \ref{method:ranker}). In second stage, at inference time, we use query performance prediction(Section\ref{method:qpp}) and routing(Section \ref{method:rank_fusion} and Section \ref{method:qpp_rf}) to get the best performance for the query using the above rankers.


\subsection{Context Aware Query Enrichment(\car{})}
\label{rewriter:method}
Consider a set of queries $Q=\{HQ \cup Q^+\}$, that comprises sets of hard queries $HQ$ and well-formed queries $Q^+$.
\begin{tcolorbox}[title= Example Prompt]
\small
\begin{minipage}{\textwidth}
\textbf{Instruction}: Being a ranking model, your first task is to do query
expansion. This means that a query and a document expand
the query so that it is relevant to the document. Expand and
contextualize the query as best as you can in one or two
short sentences.\\
\textbf{Query}: hs worms \texttt{} \\
\textbf{Context}: Established in 1996, Hochschule Worms (Worms University of Applied Sciences) is a non-profit public higher education institution 
 \dots \texttt{}
 \end{minipage}
 
% \textbf{LLM Generated Output:}

\end{tcolorbox}

Given a hard query $hq_i \in HQ$, our goal is to generate a rewritten query $q_i^*$ that enriches the original under specified query to result in a more clear and concise query for a ranker. We generate $q_i^*$ by conditioning the LLM on a few-shot prompt using the top-1 relevant document $d^+$ (from set of documents $D$) for the query. An example of a few-shot prompt employed is  shown above.
\[q_i^* = LLM(aq_i,d^+)\]

We first instruct the LLM as shown in the example above to perform the task of query enrichment in the context of the given document. We then provide an hard query ($hq_i$) concatenated with the corresponding relevant document as a part of the prompt. This \textit{context-aware prompting} of LLMs results in better rewrites without topic drifts, as the LLM is conditioned on intents conveyed in the document. We also introduce a constraint on the maximum length of the output sequence generated. This constraint coupled with grounding using document context helps prevent hallucination and topic drift.
 % We also experiment with different prompting approaches by varying the document context. We discuss the different variations of few-shot prompting and the corresponding results in Section~\ref{models} and Section~\ref{results} respectively.
% \subsubsection{Hyperparameters}
% We use a temperature of 0.5 to balance exploration and deterministic generation. We set presence penalty and frequency penalty to 0.6 and 0.8 respectively to minimize redundancy in generated reformulations of the original query. 
The resulting enriched query is used as an input to fine-tune the ranker.
Note that we only rely on LLMs to enrich hard queries for fine-tuning the ranker. During inference, the ranker directly ranks relevant documents for the new queries without the LLM based enrichment component. 

\subsubsection{Passage selector for Documents}
%\noindent \textbf{Passage selector for Documents}: 
\label{method:attention_linear}
We noticed additional \textit{topic drift} in the context of utilizing the \car{} approach with the document corpus. \textbf{Topic drift} is characterized by the divergence of a rewritten query's specificity when applying the \car{} approach to documents. This occurs due to documents encompassing multiple topics, potentially relating to one or more aspects of the query. To mitigate this occurrence of \textit{topic drift}, we employ supervised passage selection techniques (\attention{}, \linear{}) as proposed in ~\cite{leonhardt2021learnt}. These techniques aid in selecting the most relevant passage from a document, aligning it more closely with a given query.

%\subsection{Ranking Phase}
\subsection{Training Ranker}
\label{method:ranker}

 We employ the pointwise loss to train the ranker. Assume a mini batch of $N$ training examples $\left\{x_i, y_i\right\}_{i=1, ..., N}$. The ranking task is cast as a binary classification problem, where each training instance $x_i = (q^*_i, d_i)$ is a query-document pair and $y_i \in {0, 1}$ is a relevance label. The predicted score of $x_i$ is denoted as $\hat{y}_i$. The cross-entropy loss function is defined as follows:
\begin{equation}
    \mathcal{L}_{\mathtt{Point}} = -\frac{1}{N} \sum_{i=1}^{N} \left( y_{i} \cdot \log \hat{y}_{i} + (1 - y_{i}) \cdot \log (1-\hat{y}_{i}) \right)
\end{equation}

%Note that we only fine-tune the ranker on query reformulations of ambiguous or under-specified queries.
%At inference time, the ranker equipped with the knowledge of user information needs is directly deployed to rank relevant documents.
We train two rankers, one trained on hard enriched query using \car{} (Specialised ranker for Hard queries or $SR$) and the other on original queries 
 (Base Ranker or $BR$). As we generate rewrites using different LLM's, the $SR$ are thus named after their respective LLM's.


\subsection{Rank Fusion (\car{} + \rf{})}
\label{method:rank_fusion}
The $SR$ is specialized to improve the ranking performance for hard queries. To employ $SR$ for hard queries, there is a need for an effective automated way of identifying such queries during inference.
Hence, we propose to combine ranked lists from the base ranker $BR$ and the 
%ranker specialized for hard queries 
$SR$ during inference to prevent compromise in document ranking performance on other queries. We adopt the score based rank fusion approach, namely CombSUM \cite{Fox1993CombinationOM} as we observe the best performance compared to other fusion methods. More formally, for a given test query, $q_i$ and corresponding document $d_i$, 
$r_i = BR(q_i,d_i) ; r_j = SR(q_i,d_i)$
The final relevance score is calculated as the sum of document retrieval scores: $r_i+r_j$
\subsection{ Routing using Query Performance Prediction (\car{} + QPP{})}
\label{method:qpp}
While rank fusion helps us to combine the capabilities of both the models, it assigns equal weights to relevance scores from the two ranking models ($BR$ and $SR$), thereby not distinguishing hard and well-formed queries. In practice, giving higher weight to the $SR$ model score for hard queries would result in improved retrieval quality. Hence, if we have a method for determining the hard query at inference time, would choose an appropriate ranking model or assign appropriate weights to relevance scores for the rank fusion. To determine if a query is hard at inference time, we propose to fine-tune a Query Performance Prediction (QPP) model inspired by BERT-QPP \cite{bert_qpp}. Given a query $q_i$ and top-k retrieved documents $D^+_k$ for the query using BM25, we fine-tune a cross-encoder based QPP model $\psi$  using binary cross-entropy loss as follows:
\[
    \mathcal{L} = -\frac{1}{N} \sum_{i=1}^{N} \left( M(q_i,D^+) \cdot \log  \psi(q_i,D^+_k)  + 
    \\ (1 - M(q_i,D^+)) \cdot \log (1-\psi(q_i,D^+_k)) \right)
\]
where $M$ refers to nDCG score and $D^+_k$ denotes top-k relevant documents ($D^+$).

We then use a threshold decided based on range of scores estimated across queries to route the queries to $SR$ or $BR$. 
%Queries with scores below the threshold are ranked using the $SR$ and the rest using the $BR$.

\subsection{Rank Fusion using Query Performance Prediction (\car{} + QPP + \rf{})}
\label{method:qpp_rf}
Finally, we propose a QPP based rank fusion approach which combines the two ranking scores ($BR$ and $SR$) weighted by the QPP score.
%the base ranker and the ranker specialized for hard queries. 
Given a query at inference time, $q_i$ we first obtain an estimate of the query performance using the fine-tuned BERT-QPP model ($\psi$) defined in Section \ref{method:qpp} and the set of initial documents retrieved ($D^+$) using BM25.
\[qp_i = \psi\left(q_i,D^+\right)\]
Then the score is used to weigh the relevance scores obtained for the query document pairs from BR  and the SR .

\begin{equation}
    s_i = qp_i * SR(q_i,d_i) + (1-qp_i) * BR(q_i,d_i)
\label{eq:qpp_rf}
\end{equation}


The resulting score is used to rank documents. We observe that our QPP based rank fusion helps obtain better performance on hard queries without compromising performance on other queries.


==> 06-discussion.tex <==
\section{Open Questions (Remove)}
 \label{open_questions}


The proposed framework \car{} comprises a rewriter and ranker. One possible research direction is to explore end-to-end fine-tuning of the rewriter and ranker based on feedback from downstream retrieval performance. In the proposed approach \car{}, the context in the prompt is derived from the relevant document for the query. However, we observe that for longer documents, providing a concise context by truncating the original document prevents topic drift and generates concise query rewrites which reflect the user information need. One possible direction is to explore principled and automated approaches for learning to select the most relevant context for constraining the LLM outputs and guiding them to generate queries that improve document ranking performance. Existing works like active sample selection \cite{zhang-etal-2022-active} for in-context learning explores the use of RL-based approaches for selecting demonstration samples. We posit that similar approaches could be leveraged to select relevant contexts to prompt the LLM for context-aware query reformulation.

 


% \subsection{Intent Diversification}
% An overarching goal of the proposed framework is to minimize the \textit{hard rewrites} discussed in Section \ref{sec:framework}. To ensure the generative model (rewriter) generates diverse queries, the training data must ensure high \textit{intent coverage}. This implies that the dataset contains diverse intents for each query. The coverage of intents is an important consideration when selecting datasets for fine-tuning the proposed rewriter or in case of in-context learning examples. It is also vital to ensure the dataset does not contain topic drifts.
% As proposed in this work, we have leveraged several data augmentation methods based on existing large language models and TREC datasets. However, the topic descriptions in TREC are not comprehensive enough in terms of coverage of different types of intent for the same query. Additionally LLMs have been found to hallucinate \cite{hallucination}, which might lead to misconstrued machine intent in the proposed pipeline. We propose potential directions to tackle this issue.
% Dataset distillation \cite{dataset_distillation} approaches could be explored for accomplishing the selection of informative samples. This method employs several metrics from information theory for quantifying the quality of training samples. The metric is used to filter out uninformative samples yielding a succinct training set which improves performance on intended tasks. The choice of metric for query rewriting would be \textit{intent diversity}. This would be a composite metric ensuring the natural language summaries of queries are not redundant and reflect different possible intents. Further, an external Knowledge Base (KB) could be employed to ground the possible intents for each query and filter out data which deviates from the KB. Several existing approaches like REALM and LM-CORE \cite{lm_core} retrieve relevant information from knowledge based like Wikipedia and Concept-Net to aid in text completion. They could be leveraged to decipher the possible intents for an ambiguous query and compute the coverage metric. 
% Though data distillation leads to informative samples, the sample selection is limited to the training data distribution. To learn the underlying manifold of informative samples, synthetic dataset generation approaches have been proposed \cite{dataset_condensation}. These approaches aim to synthesize a smaller set that achieves similar or better performance than the default training set through gradient matching approaches.
%\vspace{-3mm}
\subsection{Limitations} In our current approach, we choose ambiguous queries based on heuristics like the query length and specific types of queries like acronyms, entities with multiple meanings based on context. Though these heuristics reflect the nature of ambiguous queries, a more principled approach would help identify and filter ambiguous queries.
\label{limitations}



==> tables/claim_datasets.tex <==
\begin{table}[htpb!]
\centering
% \footnotesize
\begin{tabular}{c c c c c}
\multicolumn{2}{c}{Claim Data} & Supporting & Non-Supporting & Total \\
\hline 
\\
\multirow{3}{*}{HoVer} & Train & 11023 (61\%) & 7148 (39\%) & 18171 \\
                       & Dev & 2000 (50\%) & 2000 (50\%) & 4000 \\
                       & Test & 2000 (50\%) & 2000 (50\%) & 4000 \\[5mm]
                       
\multirow{3}{*}{WiCE} & Train & 460 (37\%) & 800 (63\%) & 1,260 \\
                       & Dev & 115 (33\%) & 234 (67\%) & 349 \\
                       & Test & 111 (31\%) & 247 (69\%) & 358 \\[5mm]

\hline
\end{tabular}
\caption{Sizes of the claim dataset splits as used in our experiments.}
\label{tab:claim_dataset_sizes}
\end{table}

==> tables/compare_all_approach.tex <==
%\vspace{-5mm}
\begin{table*}[hbt!]
    \centering
    \begin{tabular}{lccccc}
        \toprule
            \textit{query} & \textit{is\_hard} & \textit{base\_score} & \textit{qpp\_score} & \textit{rank\_fusion} & \textit{qpp\_fusion}\\
            \midrule

eating foods that are considered warm & no & 0.114 & 0.114 & 0.504 & 0.471\\
who was the first steam boat operator & yes & 0.171 & 0.25 & 0.397 & 0.397\\
example of monotonic function & no & 0.180 & 0.180 & 0.247 & 0.283\\
what other brain proteins can cause dementia & no & 0.195 & 0.195 & 0.390 & 0.195\\
causes of military suicide & yes & 0.200 & 0.319 & 0.461 & 0.430\\
does ethambutol treat bone infection & yes & 0.291 & 0.442 & 0.414 & 0.414\\
what is chronometer who invented it & yes & 0.339 & 0.514 & 0.483 & 0.519\\
where are the benefits of cinnamon as a supplement? & yes & 0.346 & 0.559 & 0.637 & 0.559\\
how often to button quail lay eggs & yes & 0.365 & 0.441 & 0.392 & 0.413\\
anthropological definition of environment & no & 0.432 & 0.432 & 0.585 & 0.517\\
how long will methadone stay in your system & no & 0.371 & 0.371 & 0.538 & 0.653\\
how much does it cost to go to alabama university & yes & 0.671 & 0.704 & 0.704 & 0.704\\
what drives poaching & yes & 0.503 & 0.728 & 0.518 & 0.706\\
causes of gas in large intestine & no & 0.236 & 0.236 & 0.631 & 0.541\\
why does lacquered brass tarnish & yes & 0.578 & 0.684 & 0.686 & 0.765\\


        \bottomrule        
    \end{tabular}
    \caption{Comparing nDCG@10 scores for all approaches at query level. The queries are from \mshard{} document collection re-written using \chatgpt{} and \car{} method}
    \vspace{-5mm}
    \label{tab:compare_all_approaches}
\end{table*}


==> tables/feasability/feasability_datasets.tex <==
\begin{table}[hbt!]
\centering
\begin{tabular}{c|c|c|c|c}
dataset & total & train & validation & test \\
\hline
BBC XSum \cite{narayan2018dont} & 226,711 & 204,045 (90\%) & 11,332 (5\%) & 11,334 (5\%) \\
CNN/Daily Mail \cite{nallapati2016abstractive} & 311,672 & 286,817 (92\%) & 13,368 (4\%) &  11,487 (4\%) \\
MuSiQue \cite{musiqueQA} & 49,628 & 39,876 (80\%) & 4,834 (10\%) & 4,918 (10\%)  \\
2WikiMultiHopQA \cite{wikimultihopQA} & 192,606 & 167,454 (87\%) & 12,576 (6,5\%) & 12,576 (6,5\%) \\
\end{tabular}
\caption{Split sizes of the datasets into training, validation and test sets.}
\label{tab:dataset_splits}
\end{table}

==> tables/feasability/feasability_results.tex <==
\begin{table}[!htbp]
\small
\begin{tabular}{llrrrllrrr}
        & & \multicolumn{3}{c}{BBC Xsum} &  &  & \multicolumn{3}{c}{CNN/Dailymail} \\
model:  & Source: & Rouge-1 & Rouge-2 & Rouge-L &  &  & Rouge-1 & Rouge-2 & Rouge-L \\
\hline
T5-large &\cite{zhu2021leveraging} & 19.66 &  2.91 & 15.31 & & & 39.68 & 17.24 & 36.28 \\
         &\cite{rothe2021} & 44.34 & 22.01 & 36.65 &  &  & 43.59 & 21.42 & 40.56 \\
           &\cite{raffel2020} & - & - & - & &  & 42.50 & 20.68 & 39.75 \\
           & Reproduction & 40.01 & 16.61 & 32.05 &  &  & 23.96 & 6.84 & 16.56 \\
\hline
           
BART-large &\cite{zhu2021leveraging} & 26.18 &  7.60  & 20.92 &  &  & 32.83 & 13.30 & 29.64 \\
           &\cite{lewis2019bart} & 45.14 & 22.27 & 37.25 &  &  & 44.16 & 21.28 & 40.90 \\
           & Reproduction & 44.95 & 21.60 & 36.51 &  &  & 26.19 & 7.86  & 17.64                      
\end{tabular}
\caption{Rouge scores between generative models of T5 and BART and the values reported in various papers.}
\label{tab:feasability_results}
\end{table}

==> tables/feasability/qa_hallucinations.tex <==
\begin{table*}[!htbp]
\begin{tabular}{p{0.15\textwidth} p{.5\textwidth} p{.25\textwidth}}
\hline
    \textbf{Method}     & \textbf{Ouput} & \textbf{Category} \\
\hline
  \textbf{Question}  &  \textbf{What did the actress in My Fair Lady win a Tony for? [Dataset: \textbf{MQA}]} & entity hallucination due to wrong association (intrinsic) \\

GPT-3.5-turbo  & The actress in My Fair Lady who won a Tony award is \textcolor{red}{Julie Andrews}. She won the Tony for Best Actress [\dots]   \\ 

\hline
\hline
 \textbf{Question}  & \textbf{Who was born later, Gideon Johnson Pillow or Holm Jølsen?} [Dataset: \textbf{MQA}]  \\
GPT-3.5-turbo  & Gideon Johnson Pillow was born on June 8, 1806. \textcolor{red}{Holm Jølsen's birthdate is not provided.} & incomplete knowledge in parametric memory (intrinsic)  \\
 
\hline
\hline

\textbf{Question} & \textbf{What did the director of `A Stitch for Time' win at the 54th Academy Awards?} [Dataset: \textbf{MQA}] \\ 
GPT-3.5-turbo & The director of `A Stitch for Time' is \textcolor{red}{Dianne Houston}. She won the \textcolor{red}{Academy Award for Best Live Action Short Film} [...] & new entities introduced (extrinsic hallucination )\\

\hline
\hline
\textbf{Question}  & \textbf{How many students attend Daniel Thürer's university?} [Dataset: \textbf{MQA}]  \\
GPT-3.5-turbo  & \textcolor{red}{There is no information available about which university Daniel Thürer belongs to}. Therefore, it is not possible [...] & incomplete knowledge in parametric memory (intrinsic)\\

\hline
\hline
\textbf{Question} & \textbf{Who is the child of Empress Dowager Huang's child?} [Dataset: \textbf{MQA}]  \\
GPT-3.5-turbo  & Empress Dowager Huang had only one child, who was \textcolor{red}{Emperor Ai of Han}. However, Emperor Ai of Han did not have any children [...] & new entity (extrinsic hallucination) \\

\hline
\hline
\textbf{Question}  & \textbf{Do Alice Mary Dowd and Richard N. Palmer have the same nationality?} [Dataset: \textbf{WikiQA}]  \\
GPT-3.5-turbo  & \textcolor{red}{It is not specified in the given question whether Alice Mary Dowd and Richard N. Palmer have the same nationality or not.} & wrong interpretation, lack of knowledge in parametric memory  \\

\hline
\hline
\textbf{Question}  & \textbf{Where was the husband of Lou Henry Hoover born?} [Dataset: \textbf{WikiQA}]  \\
GPT-3.5-turbo  &  \textcolor{red}{Jesse Hoover}, the husband of Lou Henry Hoover, was born in Iowa. & wrong entity (intrinsic)\\

\end{tabular}
\caption{Qualitative analysis of hallucination in QA task}
\label{tab:qualitative}
%\vspace{-0.25cm}
\end{table*}

==> tables/feasability/summary_hallucinations.tex <==
\begin{table}[!htbp]
\small
\begin{tabular}{p{0.35\linewidth} p{0.3\linewidth}   p{0.3\linewidth} }
\hline
\textbf{Document text} & \textbf{Generated summary} & \textbf{Hallucination error} \\
\hline
 [...] ``He was totally up for marrying us on skis and did an amazing job. He is currently trying to establish whether or not we are the first wedding actually conducted and vowed in skis - officiate and couple " said the Reids. "We can't actually believe we are but there can't be many." [...] &  A couple who got married on skis have said they are the first to do so. & \textit{Intrinsic event-related error:} The couple does not claim they are the first to do so and even doubt it. \\
 \hline
 \hline
[...] Nigeria's Inspector General of Police  Ibrahim Idris  wants all new recruits to the country's police force to undergo a lie detector test [...] Just what sort of questions would be set for the future cops is not clear  but the move is innovative and opens up all manner of possibilities on the African political landscape in our search for the kind of public officials the continent deserves. [...]    & Nigeria's new police chief is a bold move  but one that could have implications for all African countries. 
& \textit{Intrinsic entity-related error:}  it is the inspector General of Police and not the new police chief. \newline \newline \textit{Intrinsic noun-phrase error:} The bold move should refer to the lie detector test for recruits. \\
 \hline
 \hline
 It is believed the same group of criminals are targeting Lye Valley Industrial Estate several times a week. West Midlands Police said they will put in place extra measures to help businesses. [...]    & Thieves have targeted an industrial estate in Wolverhampton  stealing more than £1m in just two weeks. & \textit{Extrinsic entity-related error:} Wolverhampton instead of Lye Valley. \newline \newline \textit{Extrinsic noun-phrase related} \textit{error:} £1m in just two weeks is not mentioned in the text. \\
 \hline
 \hline
[...] Lada's 4x4 Niva has long been the car that bucked the trend of laughing at the Russian carmaker and has won fans around the world thanks to its robust nature and chunky looks. [...] & The Russian carmaker Lada has been hailed as one of the best cars in the world. & \textit{Extrinsic event-related error:}  no mention of it being hailed as one of the best cars in the world. \\

\end{tabular}
\caption{Qualitative analysis of hallucination in Summary task}
\label{tab:characterise_hallucinations}
\end{table}

==> tables/hover/bm25/original_hover_paragraph.tex <==
\begin{table}[htpb!]

\footnotesize
\begin{tabular}{c c c c c}
    \hline
    Document Retrieval:	& results & time & Disk IO writes & \makecell[l]{max memory \\ usage} \\
    \hline
    \makecell[l]{prepare train data \\ for doc retrieval} & - & 10s59 & 212.47 MB & 665.547 MiB \\
    \makecell[l]{prepare dev data \\ for doc retrieval}	& - & 	2s44 &	47.43 MB & 164.914 MiB \\
    \makecell[l]{train BERT \\ document retrieval} & \makecell[l]{'hit5\_100': 19.65, \\'hit8\_100': 21.975, \\ 'hit10\_100': 22.9, \\ 'exact\_100': 4.425, \\ 'f1\_100': 37.778, \\ 'total\_100': 4000} & 2.28 hr (8211.47 sec) & 28.90 GB & 14148.812 MiB \\
    \makecell[l]{evaluate doc retrieval \\ for train data} &	\makecell[l]{'hit5\_900': 33.807, \\ 'hit8\_900': 35.012, \\ 'hit10\_900': 35.248, \\ 'exact\_900': 18.397, \\ 'f1\_900': 62.989, \\ 'total\_900': 18171}	& 17.64 min (1058.62 sec) & 54.36 MB & 12146.676 MiB \\
    \makecell[l]{evaluate doc retrieval \\ for dev data}	& \makecell[l]{'hit5\_900': 23.525, \\ 'hit8\_900': 25.2, \\ 'hit10\_900': 25.625, \\ 'exact\_900': 10.65, \\ 'f1\_900': 58.270, \\ 'total\_900': 4000} & 3.96 min (237.54 sec)	& - & 4700.859 MiB \\
    \hline
    Sentence Retrieval:	& results &	time & disk IO writes & max memory usage \\
    \hline
    \makecell[l]{prepare dev doc retrieval data \\ for sentence retrieval}	& - & 1.49 min (89.22 sec) & 11.27 MB& 118.340 MiB \\
   \makecell[l]{prepare train data \\ for sentence retrieval} & - &	7.33 min (439.73 sec) & 50.79 MB & 299.742 MiB \\
    \makecell[l]{train BERT \\ sentence retrieval} & \makecell[l]{'exact\_100': 0.75, \\ 'f1\_100': 14.964, \\ 'total\_100': 4000} &	3.30 hr (11868.16 sec) & 172.66 GB & 18383.195 MiB \\
    \makecell[l]{evaluate sentence \\ retrieval for train data} & \makecell[l]{'exact\_1900': 12.151, \\ 'f1\_1900': 56.408, \\ 'total\_1900': 18171}	& 4.82 min (289.14 sec) & 28.43 MB & 12094.914 MiB \\
    \makecell[l]{evaluate sentence \\ retrieval for dev data} & \makecell[l]{'exact\_1900': 4.25, \\ 'f1\_1900': 46.852, \\ 'total\_1900': 4000} & 1.14 min (68.17 sec) & - & 4400.418 MiB \\
    \hline
    Claim Verification:	& results & time & disk IO writes & max memory usage \\
    \hline
    \makecell[l]{prepare train data \\ for claim verification} &	- & 1.40 sec & 8.78 MB & 302.871 MiB \\
    \makecell[l]{prepare dev data \\ for claim verification} & - & 0.27 sec & 1.97 MB & 110.602 MiB \\
    \makecell[l]{train BERT \\ claim verification} & \makecell[l]{'acc\_100': 50.325, \\ 'total\_100': 4000}	& 14.32 min (859.21 sec) & 37.33 GB & 4381.816 MiB \\
    \makecell[l]{evaluate claim verification} & 65.875\% accuracy & 20.32 sec & - & 3727.152 MiB \\
    \hline
    Wiki db: 2.01GB &  65.875\% accuracy & 6 hours, 25 min, 56 sec & 239.90 GB & 18383.195 MiB \\
\end{tabular}
\caption{Original Hover pipeline metrics on first paragraph English Wikipedia data.}
\label{multiprogram}
\end{table}

==> tables/hover/hover_performance.tex <==
\begin{table}[htb!]
\small
\begin{tabular}{c c c c c c c c}
\multirow{2}{*}{Experiment setting} & \multirow{2}{*}{Accuracy} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{Precision} & \multicolumn{2}{c}{Recall}  \\ 
\cline{3-8}
  & &  Weighted  & Macro & Weighted & Macro & Weighted & Macro      \\
\hline
\multicolumn{1}{l}{\textit{Sparse + Re-ranking}} & & & & \\
Full-Wiki & \textbf{67.79} & \textbf{67.59} & \textbf{67.63} & \textbf{68.45} & \textbf{68.39} & \textbf{67.79}  & \textbf{67.93}\\
Claim detection & \underline{62.33} & 62.02 & 62.08 & \underline{62.98} & \underline{62.92} & \underline{62.33} & \underline{62.50} \\
Citation Extraction & 60.91 & 60.61 & 60.66 & 61.47 & 61.42 & 60.91 & 61.07 \\
Fusion & 62.28 & \underline{62.15} & \underline{62.18} & 62.60 & 62.56 & 62.28 & 62.39  \\[5mm]

\hline
\multicolumn{1}{l}{\textit{Dense Retrieval}} & & & & \\
Full-Wiki & 64.60 & 64.45 & 64.45 & 64.86 & 64.86 & 64.60 & 64.60 \\
% Original & 62.90 & 62.72 & 62.76 & 63.33 & 63.28 & 62.90 & 63.02 \\
Claim detection & \underline{61.50} & \underline{60.94} & \underline{60.94} & \underline{62.20} & \underline{62.20} & \underline{61.50} & \underline{61.50} \\
Citation Extraction & 59.67 & 59.40 & 59.46 & 60.13 & 60.09 & 59.67 & 59.82 \\
Fusion & 59.51 & 59.32 & 59.37 & 59.85 & 59.81 & 59.51 & 59.64  \\[5mm]

\hline
\multicolumn{1}{l}{\textit{Index Compression}} & & & & & & &  \\
Full-Wiki & 63.30 & 62.54 & 62.54 & 64.48 & 64.48 & 63.30 & 63.30 \\
% Original & 63.02 & 62.08 & 62.08 & 64.46 & 64.46 & 63.02 & 63.02  \\
Claim detection & \underline{61.92} & \underline{61.71} & \underline{61.71} & \underline{62.19} & \underline{62.19} & \underline{61.92} & \underline{61.93}  \\
Citation Extraction & 59.98 & 59.12 & 59.12 & 60.89 & 60.89 & 59.98 & 59.98   \\
Fusion & 61.58 & 61.43 & 61.43 & 61.75 & 61.75 & 61.58 & 61.58   \\[5mm]

\hline
\end{tabular}
\caption{Performance experiments on HoVer data and adjustments using full document text of English Wikipedia. The underlined-styled values represent the second best  within each retrieval setup.}
\label{tab:hover_performance_metrics}
\end{table}
% Full document text 
% 

==> tables/latency/bm25_latency_old.tex <==
\begin{table}[htb!]
\centering
\small
\footnotesize
\begin{tabular}{l c c c c c c c}
\multirow{2}{*}{\makecell{Methods}} & \multirow{2}{*}{Retrieval} & \multirow{2}{*}{\makecell{Re-ranking}} & \multirow{2}{*}{\makecell{Snippet \\ selection}} & \multirow{2}{*}{\makecell{Claim \\ Verification}} & \multirow{2}{*}{\makecell{Total \\ Latency}} & \multirow{2}{*}{\makecell{Speedup}} \\
& \\
\hline
\multicolumn{1}{l}{\textit{HoVer}} &  \\
 Full-Wiki & 426  ms  & 69 ms & 157  ms & 7 ms & 659 ms & - \\
Fact Extraction & 257 ms  & 71 ms & - & 10 ms & 338  ms & 1.9x \\
Citation Extraction & 246 ms  &  70 ms & - & 11 ms & 327  ms & \textbf{2.0x}  \\
Fusion & 265 ms  & 69 ms & - & 11 ms & 345  ms & 1.9x  \\

\multicolumn{1}{l}{\textit{WiCE}} & \\
  Full-Wiki &  559 ms &  77 ms &  186 ms &  9  ms  &  831  ms & - \\
Fact Extraction & 372 ms & 74 ms & - & 22 ms & 468   ms & 1.8x \\
Citation Extraction & 330 ms  & 69 ms & - & 20 ms  & 419  ms & \textbf{2.0x} \\
Fusion & 347 ms & 69 ms & - & 20 ms & 436  ms & 1.9x \\
\hline
\end{tabular}
\caption{Retrieval and total latency for Sparse retrieval with Re-ranking. Speedup is compared with respect to the total latency of the Full-Wiki setup.}
\label{tab:bm25_latency}
\vspace{-2em}
\end{table}

==> tables/latency/faiss_latency.tex <==
\begin{table}[htpb!]
\centering
\footnotesize
\begin{tabular}{l c c c c c c c c}
\multirow{2}{*}{} & \multicolumn{2}{c}{\makecell{Document retrieval}} & \multirow{2}{*}{\makecell{Sentence \\ Retrieval}} & \multirow{2}{*}{\makecell{Claim \\ Verification}} & \multicolumn{2}{c}{Total Latency} & \multicolumn{2}{c}{Speedup} \\
\cline{2-3}\cline{6-7}\cline{8-9}
& CPU & GPU &  & &  CPU & GPU & CPU & GPU \\ 
\hline
\multicolumn{1}{l}{\textit{HoVer}} &  \\
 \textbf{Full-Wiki (S+R) } &  \multicolumn{2}{c}{\textbf{491  ms}} & \textbf{157  ms} & \textbf{7 ms} &  \multicolumn{2}{c}{\textbf{659 ms}} & - & - \\

Full-Wiki & 515 ms & 31 ms & 153 ms & 8 ms & 676 ms & 192  ms & 1.0x & 3.4x \\
% Original  &  523 ms & 30 ms  & - & 9 ms & 532 ms & 39 ms & 1.2x & 16.9x \\
Claim detection & 513 ms & 23 ms & - & 8 ms & 521 ms & 31 ms & 1.3x & 21.3x  \\
Citation Extraction & 479 ms & 23 ms & - & 9 ms &  488 ms & 32 ms & 1.4x & 20.6x \\
Fusion & 500 ms  & 23 ms & - & 9 ms & 509 ms & 32  ms & 1.3x & 20.6x \\

\multicolumn{1}{l}{\textit{WiCE}} & \\
 \textbf{Full-Wiki (S+R)} & \multicolumn{2}{c}{\textbf{636 ms}} & \textbf{186 ms} & \textbf{9  ms}  & \multicolumn{2}{c}{\textbf{831  ms}} & - & - \\
Full-Wiki & 685 ms & 34 ms & 184 ms & 9 ms & 878 ms & 227  ms & 1.0x & 3.7x \\
% Original  & 610  ms & 34 ms  & - & 9 ms & 619  ms & 43 ms & 1.3x & 19.3x \\
Claim detection &  622 ms & 31 ms  & - & 9 ms & 631 ms & 40 ms & 1.3x & 20.8x \\
Citation Extraction &  610 ms & 31 ms  & - & 9 ms & 619 ms & 40 ms & 1.3x & 20.8x  \\
Fusion & 619  ms & 31 ms  & - & 9 ms & 628 ms & 40 ms & 1.3x & 20.8x  \\[5mm]
\hline
\end{tabular}
\caption{Retrieval and inference latency for Dense retrieval setup on data settings. Speedup is compared with respect to the total latency of the Sparse Retrieval setup with original data setting (bold font).}
\label{tab:faiss_latency}
\end{table}




==> tables/latency/jpq_latency.tex <==
\begin{table}[htb!]
\centering
\footnotesize
\begin{tabular}{l c c c c c c c c}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c}{\makecell{Term-based \\ document retrieval}} & \multirow{2}{*}{\makecell{Sentence \\ Retrieval}} & \multirow{2}{*}{\makecell{Claim \\ Verification}} & \multicolumn{2}{c}{Total Latency}  & \multicolumn{2}{c}{Speedup} \\
\cline{2-3}\cline{6-7}\cline{8-9}
& CPU & GPU &  & &  CPU & GPU & CPU & GPU \\ 
\hline \hline
 \multicolumn{1}{l}{\colorg\textit{HoVer}} & \colorg & \colorg & \colorg & \colorg & \colorg & \colorg & \colorg & \colorg \\
 \textbf{Full-Wiki (S+R)} &  \multicolumn{2}{c}{\textbf{491  ms}} & \textbf{157  ms} & \textbf{7 ms} &  \multicolumn{2}{c}{\textbf{659 ms}} & - & - \\
Full-Wiki &  53 ms & 13 ms & 153 ms & 8 ms & 214  ms & 174 ms & 3.1x &  3.8x \\
% Original  &  55 ms & 13 ms  & - & 12 ms & 67 ms & 25 ms & 9.8x &  26.4x \\
Claim detection  &  51 ms & 12  ms  & - &  9 ms & 60 ms & 21 ms & 11.0x & 31.4x  \\
Citation Extraction  & 46  ms & 11 ms  & - & 9 ms & 51 ms & 20 ms & 12.9x & 33.0x \\
Fusion  & 51  ms & 12 ms  & - & 12 ms & 63 ms & 24 ms &  10.5x & 27.5x \\
\hline
\multicolumn{1}{l}{\colorg\textit{WiCE}} & \colorg & \colorg & \colorg & \colorg & \colorg & \colorg & \colorg & \colorg  \\
 \textbf{Full-Wiki (S+R)} & \multicolumn{2}{c}{\textbf{636 ms}} & \textbf{186 ms} & \textbf{9  ms}  & \multicolumn{2}{c}{\textbf{831  ms}} & - & - \\
Full-Wiki & 97 ms & 43 ms & 186 ms & 9 ms & 292 ms & 238 ms & 2.8x  &  3.5x \\
% Original  &  95 ms & 43  ms  & - & 11 ms & 106 ms & 54 ms & 7.8x &  15.4x \\
Claim detection  &  92 ms & 37 ms  & - & 11 ms & 103 ms & 48 ms & 8.1x & 17.3x \\
Citation Extraction  & 89  ms & 37 ms  & - & 9 ms & 98 ms & 46 ms & 8.5x & 18.1x \\
Fusion  & 89  ms & 37  ms  & - &  9 ms & 98 ms & 46  ms & 8.5x &  18.1x \\
\hline
\end{tabular}
\caption{Retrieval and inference latency for Index compression setup. Speedup is compared to the total latency of (S+R) pipeline with Full-Wiki setup.}
\label{tab:jpq_latency}
\vspace{-2em}
\end{table}


==> tables/literature/hallucination_errors.tex <==
\begin{table}[ht]
    \small
    \begin{tabular}{p{0.25\textwidth}  p{0.25\textwidth}   p{0.4\textwidth} }
    Error type & Hallucination type & Explanation\\
    \hline
    \multirow{2}{*}{Entity-related}  & Intrinsic & Incorrectly combining distinct entities from the source text.  \\
                                     & Extrinsic & Introducing new entities not present in the source text.   \\[7mm]

    \multirow{2}{*}{Event-related}   & Intrinsic & Mixing up attributes from the source text. \\
                                     & Extrinsic & Introducing new events not present in the source text. \\[7mm]

    \multirow{2}{*}{Noun Phrase-related}  & Intrinsic & Combining with the wrong modifier from the source text. \\
                                         & Extrinsic & Hallucinating new noun-phrase modifiers. \\[5mm]

    Other & \textit{Not Applicable} & Ungrammatical text, repeated words, highly erroneous spans, etc. in general what does not fit the above categories. \\
    \hline
    \end{tabular}
    \caption{Error categories for generated text further divided by hallucination categories of Intrinsic and Extrinsic nature.}
    \label{tab:hallucination_errors}
\end{table}

==> tables/live_factcheck/latency_live_factchecking_old.tex <==
\begin{table}[htb!]
\centering
\footnotesize % Reduced font size
\setlength{\tabcolsep}{3pt} % Reduce space between columns
\renewcommand{\arraystretch}{0.9} % Reduce space between rows
\begin{tabular}{l c c c c c c c c C}
\multirow{2}{*}{\makecell{Experiment \\ Setting}} & \multicolumn{2}{c}{\makecell{ Document  \\ Retrieval}} & \multirow{2}{*}{\makecell{ Document \\ Ranking}} & \multirow{2}{*}{\makecell{Sentence \\ Retrieval}} & \multirow{2}{*}{\makecell{Claim \\ Verification}} & \multicolumn{2}{c}{Total Latency} & \multicolumn{2}{c}{Speedup} \\
\cline{2-3}\cline{7-10} \\[-1mm]
& CPU & GPU & & & & CPU & GPU & CPU & GPU \\
\hline \\

% Term-based Document Retrieval
\multicolumn{10}{l}{\textit{Sparse + Re-ranking}} \\ 
\textbf{Full-Wiki} & \textbf{463 ms} & - & \textbf{107 ms} & \textbf{93 ms} & \textbf{32 ms} & \textbf{695 ms} & - & \multicolumn{2}{c}{-} \\
Fusion & 274 ms & - & 96 ms & - &  109 ms & 479  ms & - & \multicolumn{2}{c}{1.5x} \\
\hline \\
% Dense Retrieval setup
\multicolumn{10}{l}{\textit{Dense Retrieval}} \\ 
Full-Wiki &  433 ms & 32  ms & - & 88 ms & 32 ms & 553  ms &  152 ms & 1.3x & 4.6x \\
Fusion & 412  ms & 32  ms & - & - & 99 ms & 511 ms & 131 ms & 1.4x & 5.3x \\
\hline \\
% Index Compression setup
\multicolumn{10}{l}{\textit{Index Compression}} \\ 
Full-Wiki & 100 ms & 50 ms & - & 96 ms & 32 ms & 228 ms & 178 ms & 3.0x & 3.9x \\
Fusion & 89 ms & 43 ms & - & - & 114 ms & 203 ms & 157 ms & 3.4x & 4.4x \\

\hline
\end{tabular}
\caption{Latency and Speedup Comparisons Across Different Retrieval Setups for Live Fact-checking}
\label{tab:combined_latency}
\end{table}



==> tables/live_factcheck/performance_comparison_live_factcheck.tex <==
\begin{table*}[htb!]
\centering
\footnotesize
\begin{tabular}{c c c c c c c c}
\multirow{2}{*}{Experiment setting} & \multirow{2}{*}{Accuracy} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{Precision} & \multicolumn{2}{c}{Recall}  \\ 
\cline{3-8}
  & &  Weighted  & Macro & Weighted & Macro & Weighted & Macro      \\
\hline
\multicolumn{1}{l}{\colorg\textit{Sparse + Re-ranking}} & \colorg & & & \\
Full-Wiki & 56.94 & 56.95 & 56.72 & 56.96 & 56.72 & 56.94 & 56.72  \\
Fusion & 56.23 & 55.92 & 55.50 & 55.94 & 55.74 & 56.23 & 55.58  \\

\hline
\multicolumn{1}{l}{\textit{Dense Retrieval}} & & & & \\
Full-Wiki & 57.65 & 56.66 & 56.03 & 57.30 & 57.18 & 57.65 & 56.53  \\
Fusion & 58.36 & 57.82 & 57.32 & 58.06 & 57.92  & 58.36 & 57.51 \\

\hline
\multicolumn{1}{l}{\textit{Index Compression}} & & & & & & &  \\
Full-Wiki  & 57.65 & 56.94 & 56.38  &  57.30 & 57.16 & 57.65 & 56.69 \\
% Fusion & 52.67 & 52.55 & 52.19  & 52.50 & 52.24 & 52.67 & 52.22  \\[5mm]
Fusion & 53.02 & 52.93 & 52.59  & 52.88 & 52.62 & 53.02 & 52.60  \\
\hline
\end{tabular}
\caption{Live fact checking case study: Kamala Harris Vs Donald Trump debate.}
\label{tab:live_fact_check_performance_metrics}
\vspace{-2em}
\end{table*}


==> tables/rank_fusion_msmarco.tex <==
%\vspace{-5mm}
\begin{table*}[hbt!]
    \centering
    \begin{tabular}{lll|ll}
        \toprule
            %\multicolumn{5}{c}{\textbf{\trecdl{}}}\\
            % \midrule
                & \multicolumn{2}{l}{\textbf{\trecdl{}-Document}} & \multicolumn{2}{l}{\textbf{\trecdl{}-Passage}}\\
             \midrule
            %\textit{Ranking Models} & \multicolumn{1}{c}{\textbf{19}} & \multicolumn{1}{c}{\textbf{20}} & \multicolumn{1}{c}{\textbf{19}} & \multicolumn{1}{c}{\textbf{20}}\\
            \textit{Ranking Models}
             &  $\textbf{19}$ & $\textbf{20}$ & $\textbf{19}$ & $\textbf{20}$\\
            \midrule


\multicolumn{5}{l}{\bf Baselines} \\
\bert{} Baseline (BR)& 0.616 & 0.600  & 0.687 & 0.673 \\
\qd{} \cite{wang2023query2doc} & 0.613\up{1.2} & 0.606\up{1}  & 0.688\up{0.3} & 0.655\down{2.8} \\
\ct{} \cite{jagerman2023query} & 0.590\down{4.3}$^{*}$ & 0.599\up{0}  & 0.667\down{2.9}$^{\#}$& 0.693\up{2.9}\\
%hard baseline & 0.517\down{16}$^{*}$ & 0.504\down{15.9}$^{*}$ & 0.494\down{28}$^{*}$& 0.383\down{43.1}$^{*}$\\
%\vinci{} (ICL) & 0.629\up{2.1}$^{\#}$ & 0.603\up{0.5}$^{\#}$ & 0.699\up{1.9}$^{\#}$ & 0.674\up{0.1}$^{*}$ \\
%\midrule
%\multicolumn{5}{l}{\bf Query expansion + Rank Fusion} \\
%\bart{} (topic) & - & -   &&  - & 0.689\up{2.4} \\
%\ada{} & - & -  &  & 0.691\up{0.7} & 0.686\up{1.9}
%\babbage{} & - & -   &  & 0.701\up{2.1} & 0.679\up{0.8}
%\curie{} & - & -  && 0.699\up{1.8} & 0.683\up{1.5} \\
%\davinci{} & - & - && 0.698\up{1.7} & 0.682\up{1.3} \\
%\vinci{} (prompt1) & - & - &  & 0.698\up{1.7} & 0.678\up{0.7}
%\vinci{}(prompt2) & - & - &  & 0.696\up{1.3} & 0.693\up{2.9}
%\vinci{} & 0.629\up{2.1} & 0.603\up{0.5} && 0.699\up{1.9} & 0.674\up{0.1} \\
%\chatgpt{} & - & - && 0.704\up{2.5} & 0.691\up{2.6} \\
\midrule

\multicolumn{5}{l}{\bf \car{}} \\
Oracle & 0.658\up{6.8} & 0.626\up{4.4}& 0.708\up{3.1}& 0.697\up{3.5}\\
\vinci{} ($\car{}_{BRF}$)& 0.622\up{1}$^{\#}$ & \textbf{0.618\up{3.1}}$^{\#}$ & \textbf{0.700\up{2.0}}$^{*}$ & \textbf{0.690\up{2.5}}$^{*}$ \\
\vinci{} ($\car{}_{QPP}$)& 0.622\up{1.1}$^{\#}$ & 0.610\up{1.7}$^{\#}$ & 0.696\up{1.3}$^{*}$ & 0.689\up{2.3}$^{\#}$ \\
\vinci{} ($\car{}_{WRF}$) & \textbf{0.625\up{1.5}}$^{*}$ & 0.590\down{1.7}$^{*}$ & 0.679\down{1.0}$^{\#}$ & 0.665\down{1.2}$^{*}$ \\

%\multicolumn{5}{l}{\bf \car{} + Rank Fusion} \\
%\bart{} (topic+PAA) & 0.622\up{0.9} & 0.605\up{0.8} && 0.69\up{0.6} & 0.686\up{1.9} \\
%\vinci{} & 0.63\up{2.3} & 0.603\up{0.6} && 0.700\up{1.9} & 0.690\up{2.5} \\
%\chatgpt{} & 0.626\up{1.6} & 0.609\up{1.6} && 0.708\up{3.1} & 0.693\up{2.9} \\
%\vinci{} (\attention{}) & 0.629\up{2.2} & 0.61\up{1.7} && - & - \\
%\vinci{} (\linear{}) & 0.622\up{1} & 0.618\up{3.1} && - & - \\
%\chatgpt{} (\attention{}) & 0.618\up{0.4} & 0.608\up{1.3} && - & - \\
%\chatgpt{} (\linear{}) & 0.633\up{2.8} & 0.605\up{0.9}  && - & - \\

%\midrule
%\multicolumn{5}{l}{\bf \car{} + QPP} \\
%\bart{} (topic+PAA) & 0.626\up{1.7} & 0.605\up{0.8} &  & 0.688\up{0.2} & 0.683\up{1.5} \\
%\vinci{} & 0.621\up{0.9} & 0.608\up{1.3} &  & 0.696\up{1.3} & 0.689\up{2.3} \\
%\chatgpt{} & 0.620\up{0.6} & 0.602\up{0.3} &  & 0.703\up{2.4} & 0.690\up{2.5} \\
%\vinci{} (\attention{}) & 0.624\up{1.4} & 0.605\up{0.8} &  &  &  \\
%\vinci{} (\linear{}) & 0.625\up{1.5} & 0.603\up{0.5} &  &  & \\
%\chatgpt{} (\attention{}) & 0.622\up{1.1} & 0.61\up{1.7} &  &  & \\
%\chatgpt{} (\linear{}) & 0.624\up{1.4} & 0.607\up{1.2} &  &  & \\
%\midrule
%\multicolumn{5}{l}{\bf \car{} + QPP + Rank Fusion} \\
%\bart{}(topic+PAA) & 0.620\up{0.7} & 0.584\down{2.6} &  & 0.657\down{4.3} & 0.670\down{0.5} \\
%\vinci{} & 0.625\up{1.5} & 0.590\down{1.7} &  & 0.679\down{-1.0} & 0.665\down{1.2} \\
%\chatgpt{}  & 0.618\up{0.4} & 0.582\down{3.1} && 0.687\up{0.0} & 0.657\down{2.4} \\
%\vinci{} (\attention{}) & 0.624\up{1.3} & 0.5874\down{2.1} &  &  &  \\
%\vinci{} (\linear{}) & 0.615\down{0.1} & 0.583\down{2.8} &  &  & \\
%\chatgpt{} (\attention{}) & 0.609\down{1.1} & 0.592\down{1.3} &  &  & \\
%\chatgpt{} (\linear{}) & 0.607\down{1.5} & 0.589\down{1.8} &  &  & \\

        \bottomrule        
    \end{tabular}
    \caption{Comparison between Baseline (BR) and our approaches ($\car{}_{BRF}$, $\car{}_{QPP}$, $\car_{WRF}$) on \trecdl{}-19 and \trecdl{}-20, Passage and Document sets. Relative improvement of approaches against a baseline (BR) in parentheses. Statistically significant improvements at a level of $95\%$ and $90\%$ are indicated by $*$ and $\#$ respectively~\cite{paired_significance_test}. The best results for dataset is in \textbf{bold}.}
    \vspace{-5mm}
    \label{tab:rank_fusion_msmarco}
\end{table*}


==> tables/rank_fusion_msmarco_bck.tex <==
\begin{table*}[hbt!]
    \centering
    \begin{tabular}{llcc|cc}
        \toprule
            & \multicolumn{5}{c}{\textbf{\trecdl{}}}\\
             \midrule
            & \multicolumn{2}{c}{\textbf{Document}} && \multicolumn{2}{c}{\textbf{Passage}}\\
             \midrule
            \textit{Ranking Models} & \multicolumn{1}{c}{\textbf{19}} & \multicolumn{1}{c}{\textbf{20}} && \multicolumn{1}{c}{\textbf{19}} & \multicolumn{1}{c}{\textbf{20}}\\
            \midrule


\multicolumn{5}{l}{\bf Baseline} \\
\bert{} Baseline & 0.616 & 0.6  && 0.687 & 0.673 \\
\qd{} & 0.613\up{1.2} & 0.606\up{1}  && 0.6883\up{0.26} & 0.655\down{2.8} \\
\midrule
\multicolumn{5}{l}{\bf Query expansion + Rank Fusion} \\
\bart{} (topic) & - & -   &&  - & 0.689\up{2.4} \\
%\ada{} & - & -  &  & 0.691\up{0.7} & 0.686\up{1.9}
%\babbage{} & - & -   &  & 0.701\up{2.1} & 0.679\up{0.8}
\curie{} & - & -  && 0.699\up{1.8} & 0.683\up{1.5} \\
\davinci{} & - & - && 0.698\up{1.7} & 0.682\up{1.3} \\
%\vinci{} (prompt1) & - & - &  & 0.698\up{1.7} & 0.678\up{0.7}
%\vinci{}(prompt2) & - & - &  & 0.696\up{1.3} & 0.693\up{2.9}
\vinci{} & 0.629\up{2.1} & 0.603\up{0.5} && 0.699\up{1.9} & 0.674\up{0.1} \\
\chatgpt{} & - & - && 0.704\up{2.5} & 0.691\up{2.6} \\
\midrule
\multicolumn{5}{l}{\bf \car{} + Rank Fusion} \\
\bart{} (topic+PAA) & 0.622\up{0.9} & 0.605\up{0.8} && 0.69\up{0.6} & 0.686\up{1.9} \\
\vinci{} & 0.63\up{2.3} & 0.603\up{0.6} && 0.700\up{1.9} & 0.690\up{2.5} \\
\chatgpt{} & 0.626\up{1.6} & 0.609\up{1.6} && 0.708\up{3.1} & 0.693\up{2.9} \\
\vinci{} (\attention{}) & 0.629\up{2.2} & 0.61\up{1.7} && - & - \\
\vinci{} (\linear{}) & 0.622\up{1} & 0.618\up{3.1} && - & - \\
\chatgpt{} (\attention{}) & 0.618\up{0.4} & 0.608\up{1.3} && - & - \\
\chatgpt{} (\linear{}) & 0.633\up{2.8} & 0.605\up{0.9}  && - & - \\

\midrule
\multicolumn{5}{l}{\bf \car{} + QPP} \\
\bart{} (topic+PAA) & 0.626\up{1.7} & 0.605\up{0.8} &  & 0.688\up{0.2} & 0.683\up{1.5} \\
\vinci{} & 0.621\up{0.9} & 0.608\up{1.3} &  & 0.696\up{1.3} & 0.689\up{2.3} \\
\chatgpt{} & 0.620\up{0.6} & 0.602\up{0.3} &  & 0.703\up{2.4} & 0.690\up{2.5} \\
\vinci{} (\attention{}) & 0.624\up{1.4} & 0.605\up{0.8} &  &  &  \\
\vinci{} (\linear{}) & 0.625\up{1.5} & 0.603\up{0.5} &  &  & \\
\chatgpt{} (\attention{}) & 0.622\up{1.1} & 0.61\up{1.7} &  &  & \\
\chatgpt{} (\linear{}) & 0.624\up{1.4} & 0.607\up{1.2} &  &  & \\
\midrule
\multicolumn{5}{l}{\bf \car{} + QPP + Rank Fusion} \\
\bart{}(topic+PAA) & 0.620\up{0.7} & 0.584\down{2.6} &  & 0.657\down{4.3} & 0.670\down{0.5} \\
\vinci{} & 0.625\up{1.5} & 0.590\down{1.7} &  & 0.679\down{-1.0} & 0.665\down{1.2} \\
\chatgpt{}  & 0.618\up{0.4} & 0.582\down{3.1} && 0.687\up{0.0} & 0.657\down{2.4} \\
\vinci{} (\attention{}) & 0.624\up{1.3} & 0.5874\down{2.1} &  &  &  \\
\vinci{} (\linear{}) & 0.615\down{0.1} & 0.583\down{2.8} &  &  & \\
\chatgpt{} (\attention{}) & 0.609\down{1.1} & 0.592\down{1.3} &  &  & \\
\chatgpt{} (\linear{}) & 0.607\down{1.5} & 0.589\down{1.8} &  &  & \\

        \bottomrule        
    \end{tabular}
    \caption{The results of Rank Fusion methods for TRECDL 19 and TRECDL 20 on Passage and Document test sets, with percentage improvements relative to the baseline model (Non Rank Fusion) indicated.}
    \vspace{-5mm}
    \label{tab:rank_fusion_msmarco}
\end{table*}


==> tables/ranking_msmarco_hard_doc_pass.tex <==
%\vspace{-5mm}
\begin{table*}
    \centering
    \begin{tabular}{lll|ll}
        \toprule

             %\multicolumn{5}{c}{\textbf{\mshard{}}} \\
             %\midrule
             & \multicolumn{2}{l}{\textbf{Document}} & \multicolumn{2}{l}{\textbf{Passage}}\\
             \midrule
             \textit{Ranking Models}
             &  $\text{RR}$ & $\text{nDCG}_\text{10}$ & $\text{RR}$ & $\text{nDCG}_\text{10}$\\
            \midrule


\multicolumn{3}{l}{\bf Baselines} \\
BM25+\bert{}-base (BR) & 0.444 & 0.324 & 0.5118 & 0.357\\	
\qd{}~\cite{wang2023query2doc} & 0.510\up{14.9}& 0.248\down{23.5}$^{*}$ & 0.483\down{5.6}$^{*}$& 0.284\down{20.5}$^{*}$ \\
\ct{} \cite{jagerman2023query} & 0.566\up{27.5}& 0.336\up{3.7}$^{\#}$& 0.629\up{22.9}$^{\#}$ & 0.37\up{3.7}$^{\#}$\\
\midrule
\multicolumn{3}{l}{\bf Other Baselines} \\
BM25 & 0.368 \down{17.1} &  0.272 \down{16} & 0.504 \down{1.5} & 0.304\down{14.9} \\
%BM25+RM3 &  0.365 \down{17.8} &  0.279\down{13.8} & 0.409\down{20.1} & 0.273\down{23.5} \\
BERT-MaxP(ZS) & 0.405\down{8.8} & 0.310\down{4.3} & 0.558\up{9} & \underline{0.399\up{11.8}} \\
BERT-MaxP  & 0.402\down{9.5} & 0.317\down{2.1}& - & - \\
RM3+BERT-MaxP(ZS)~\cite{lavrenko2017relevance}  & 0.415\down{6.5} & 0.314\down{3} & 0.559\up{9.2} & 0.395\up{10.6} \\
RM3+BERT-MaxP~\cite{lavrenko2017relevance} & 0.443\down{0.2} & 0.295\down{8.9}& - & - \\
T5-MaxP(ZS)~\cite{raffel2020exploring}  & 0.367\down{17.3} &  0.327\up{1} & 0.591\up{15.5} & \textbf{0.408\up{14.3}}\\
RM3+T5-MaxP(ZS)~\cite{raffel2020exploring} & 0.359\down{19.1} &  0.307\down{5.2} & 0.577\up{12.7} & 0.396\up{10.9}\\
Electra-MaxP~\cite{clark2020electra} & 0.448\up{0.9} & 0.385\up{18.9}& - & - \\
RM3+Electra-MaxP~\cite{clark2020electra} & 0.461\up{3.8} &  0.380\up{ 17.4}& - & - \\
PARADE-BERT~\cite{li2020parade} & 0.413\down{7.0} & 0.299\down{7.7}& - & - \\
RM3+PARADE-BERT~\cite{li2020parade} &  0.419\down{5.6} & 0.313\down{3.3}& - & - \\
PARADE-Electra~\cite{li2020parade}~\cite{clark2020electra} & 0.498\up{12.2} & 0.356\up{9.9}& - & - \\
RM3+PARADE-Electra~\cite{li2020parade}~\cite{clark2020electra} & 0.489\up{10.1} & 0.357\up{10.3}& - & - \\
\midrule
\multicolumn{3}{l}{\bf Oracle} \\
 $\bart{}_{paa}$ & 0.715\up{61.0} & 0.376\up{16.2} & 0.646\up{26.2} & 0.388\up{8.6}\\
\vinci{}  & 0.771\up{73.6} & 0.396\up{22.2} & 0.637\up{24.5} & 0.397\up{11.2}\\
\chatgpt{}  & 0.763\up{71.9} & 0.390\up{20.5} & 0.657\up{28.5} & 0.394\up{10.4}\\
\midrule
\multicolumn{3}{l}{\bf $\car{}_{BRF}$} \\
 $\bart{}_{paa}$ & 0.543\up{22.3} & 0.340\up{5.1}$^{\#}$ & 0.533\up{4.2} & 0.370\up{3.5} \\
\vinci{} &  0.499\up{12.4}$^{*}$ & 0.368\up{13.8}$^{*}$ & 0.551\up{7.6}$^{*}$ & 0.378\up{5.7}$^{*}$ \\
\chatgpt{} & 0.535\up{20.5}$^{*}$ & 0.368\up{13.7}$^{\#}$ & 0.555\up{8.5}$^{\#}$ & 0.381\up{6.8}$^{*}$\\
%\vinci{}(\attention{}) & 0.524\up{18.1} & 0.363\up{12}& - & - \\
%\vinci{}(\linear{}) & 0.557\up{25.5} &  0.353\up{9}& - & - \\
%\chatgpt{}(\attention{}) & 0.535\up{20.5} & 0.368\up{13.7}& - & - \\
%\chatgpt{}(\linear{}) &  0.525\up{18.3} & 0.364\up{12.5}& - & - \\


\midrule
\multicolumn{3}{l}{\bf $\car{}_{QPP}$} \\
 $\bart{}_{paa}$ & 0.575\up{29.5} & 0.356\up{9.9}$^{\#}$ & 0.631\up{23.3} & 0.376\up{5.2}\\
\vinci{} & 0.598\up{34.6}$^{*}$ & 0.366\up{13.0}$^{\#}$ & 0.628\up{22.8}$^{*}$ & 0.381\up{6.8}$^{*}$ \\
%\vinci{} llm & 0.628\up{41.5} & 0.352\up{8.7}& & \\
\chatgpt{} & 0.618\up{39.3}$^{*}$ & \underline{0.382\up{17.9}}$^{*}$ & 
\underline{0.637\up{24.4}}$^{\#}$ & 0.384\up{7.5}$^{\#}$ \\
%\chatgpt{} llm & 0.610\up{37.3}$^{*}$ & 0.346\up{6.9} & &  \\
%\vinci{}(\attention{}) & 0.763\up{71.8} & 0.366\up{13.0} & - & - \\
%\vinci{}(\linear{}) & 0.723\up{62.7} & 0.362\up{11.7} & - & -\\
%\chatgpt{}(\attention{}) & 0.688\up{54.9} & 0.36\up{11.3} & - & - \\
%\chatgpt{}(\linear{}) &  0.74\up{66.7} & \underline{0.382\up{17.9}} & - & - \\
%\midrule
%\multicolumn{3}{l}{\bf \car{} + QPP(LLM) } \\
%\bart{} (paa) & & &  & \\
%\vinci{} llm & 0.628\up{41.5} & 0.352\up{8.7}& & \\
%\chatgpt{} llm & 0.610\up{37.3}$^{*}$ & 0.346\up{6.9} & &  \\
\midrule
\multicolumn{3}{l}{\bf $\car_{WRF}$} \\
 $\bart{}_{paa}$ & 0.617\up{39.1} & 0.353\up{9.1} & 0.580\up{13.3} & 0.342\down{4.2}$^{\#}$\\
\vinci{} & \underline{0.626\up{41}} & 0.374\up{15.6}$^{*}$ & 0.623\up{21.8}$^{*}$ & 0.363\up{1.7}$^{\#}$ \\
%\vinci{}llm & 0.684\up{54} & 0.375\up{15.8} &  &  \\
\chatgpt{} & \textbf{0.659\up{48.4}}$^{\#}$ & \textbf{0.389\up{20.2}}$^{*}$ & \textbf{0.64\up{25}}$^{\#}$ & 0.380\up{6.4}$^{*}$ \\
%\chatgpt{} llm &0.638\up{43.6}& 0.364\up{12.5} &  &  \\
%\vinci{}(\attention{}) & 0.654\up{47.4} & 0.367\up{13.4} & - & - \\
%\vinci{}(\linear{}) & 0.659\up{48.5} & 0.354\up{9.4} & - & -\\
%\chatgpt{}(\attention{}) & 0.749\up{68.6} & \textbf{0.389\up{20.2}} & - & - \\
%\chatgpt{}(\linear{}) & 0.67\up{51} & 0.365\up{12.6} & - & - \\

\bottomrule        
    \end{tabular}

    \caption{\small{Comparison between Baselines and our approaches ($\car{}_{BRF}$, $\car{}_{QPP}$, $\car_{WRF}$) on \mshard{}. We show the relative improvement of approaches against a baseline (BR) in parentheses. Statistically significant improvements at a level of $95\%$ and $90\%$ are indicated by $*$ and $\#$ respectively~\cite{paired_significance_test}. The best results for dataset is in \textbf{bold} and second is \underline{underlined}.}}
    \vspace{-15mm}
    \label{tab:reranking-msmarco-hard-doc}
\end{table*}


==> tables/ranking_msmarco_hard_doc_pass_bck.tex <==
% \vspace{-15mm}
\begin{table}
    \centering
    \begin{tabular}{lcc|cc}
        \toprule

             \multicolumn{5}{c}{\textbf{\mshard{}}} \\
             \midrule
             \multicolumn{2}{c}{\textbf{Document}} && \multicolumn{2}{c}{\textbf{Passage}}\\
             \midrule
             \textit{Ranking Models}
             &  $\text{RR}$ & $\text{nDCG}_\text{10}$ & $\text{RR}$ & $\text{nDCG}_\text{10}$\\
            \midrule


\multicolumn{3}{l}{\bf Baseline} \\
Baselines(BM25+\bert{}-base) & 0.444 & 0.324 & 0.5118 & 0.357\\	
\qd{} & 0.510\up{14.9}& 0.248\down{23.5} & 0.483\down{5.6}& 0.284\down{20.5} \\
\midrule
\multicolumn{3}{l}{\bf Other Baselines} \\
BM25 &  0.368 \down{17.1} &  0.272 \down{16} & 0.504 \down{1.5} & 0.304\down{14.9} \\
%BM25+RM3 &  0.365 \down{17.8} &  0.279\down{13.8} & 0.409\down{20.1} & 0.273\down{23.5} \\
BERT-MaxP(Zero-Shot) & 0.405\down{8.8} & 0.31\down{4.3} & 0.558\up{9} & 0.399\up{11.8} \\
BERT-MaxP  & 0.402\down{9.5} & 0.317\down{2.1}& - & - \\
RM3+BERT-MaxP(Zero-Shot) & 0.415\down{6.5} & 0.314\down{3} & 0.559\up{9.2} & 0.395\up{10.6} \\
RM3+BERT-MaxP & 0.443\down{0.2} & 0.295\down{8.9}& - & - \\
T5-MaxP(Zero-Shot)& 0.367\down{17.3} &  0.327\up{1} & 0.591\up{15.5} & 0.408\up{14.3}\\
RM3+T5-MaxP(Zero-Shot)& 0.359\down{19.1} &  0.307\down{5.2} & 0.577\up{12.7} & 0.396\up{10.9}\\
Electra-MaxP & 0.448\up{0.9} & 0.385\up{18.9}& - & - \\
RM3+Electra-MaxP & 0.461\up{3.8} &  0.38\up{ 17.4}& - & - \\
PARADE-BERT &  0.413\down{7} & 0.299\down{7.7}& - & - \\
RM3+PARADE-BERT &  0.419\down{5.6} & 0.313\down{3.3}& - & - \\
PARADE-Electra & 0.498\up{12.2} & 0.356\up{9.9}& - & - \\
RM3+PARADE-Electra & 0.489\up{10.1} & 0.357\up{10.3}& - & - \\
\midrule
\multicolumn{3}{l}{\bf \car{} + Rank Fusion} \\
\bart{} (paa) & 0.543\up{22.3} & 0.340\up{5.1} & 0.533\up{4.2} & 0.370\up{3.5} \\
\vinci{} &  0.499\up{12.4} & 0.368\up{13.8} & 0.551\up{7.6} & 0.378\up{5.7} \\
\chatgpt{} & 0.482\up{8.5}  & 0.356\up{10} & 0.555\up{8.5} & 0.381\up{6.8}\\
\vinci{}(\attention{}) & 0.524\up{18.1} & 0.363\up{12}& - & - \\
\vinci{}(\linear{}) & 0.557\up{25.5} &  0.353\up{9}& - & - \\
\chatgpt{}(\attention{}) & 0.535\up{20.5} & 0.368\up{13.7}& - & - \\
\chatgpt{}(\linear{}) &  0.525\up{18.3} & 0.364\up{12.5}& - & - \\

\midrule
\multicolumn{3}{l}{\bf \car{} + QPP } \\
\bart{} (paa) & 0.727\up{63.7} & 0.356\up{9.9} & 0.631\up{23.3} & 0.376\up{5.2}\\
\vinci{} & 0.642\up{44.6} & 0.349\up{7.6} & 0.628\up{22.8} & 0.381\up{6.7} \\
\chatgpt{} & 0.862\up{94.3} & 0.380\up{17.3} & 0.637\up{24.4} & 0.384\up{7.5} \\
\vinci{}(\attention{}) & 0.763\up{71.8} & 0.366\up{13.0} & - & - \\
\vinci{}(\linear{}) & 0.723\up{62.7} & 0.362\up{11.7} & - & -\\
\chatgpt{}(\attention{}) & 0.688\up{54.9} & 0.36\up{11.3} & - & - \\
\chatgpt{}(\linear{}) &  0.74\up{66.7} & \underline{0.382\up{17.9}} & - & - \\

\midrule
\multicolumn{3}{l}{\bf \car{} + QPP + Rank Fusion} \\
\bart{} (paa) & 0.681\up{53.4} & 0.353\up{9.1} & 0.580\up{13.3} & 0.342\down{4.2}\\
\vinci{} & 0.721\up{62.3} & 0.374\up{15.6} & 0.623\up{21.8} & 0.363\up{1.7} \\
\chatgpt{} & 0.682\up{53.7} & 0.357\up{10.4} & 0.64\up{25} & 0.38\up{6.4} \\
\vinci{}(\attention{}) & 0.654\up{47.4} & 0.367\up{13.4} & - & - \\
\vinci{}(\linear{}) & 0.659\up{48.5} & 0.354\up{9.4} & - & -\\
\chatgpt{}(\attention{}) & 0.749\up{68.6} & \textbf{0.389\up{20.2}} & - & - \\
\chatgpt{}(\linear{}) & 0.67\up{51} & 0.365\up{12.6} & - & - \\

\bottomrule        
    \end{tabular}

    
    \caption{Comparison between Baseline, our approach with Rank Fusion and our approach with QPP on \mshard{}.}
    \vspace{-5mm}
    \label{tab:reranking-msmarco-hard-doc}
\end{table}


==> tables/ranking_msmarco_hard_pass.tex <==
\begin{table}
    \centering
    \begin{tabular}{lcc}
        \toprule

             \multicolumn{3}{c}{\textbf{\mshard{} Passage}} \\
            \cmidrule(lr){1-3}
            \textit{Ranking Models}
            &    $\text{RR}$ & $\text{nDCG}_\text{10}$ \\
            \midrule

\multicolumn{3}{l}{\bf Baseline} \\
Baselines(BM25+BERT rank) & 0.5118 & 0.357\\
\midrule
\multicolumn{3}{l}{\bf Other Baselines} \\
BM25 & 0.504 & 0.304\\
BM25+RM3 & 0.409 & 0.273\\
BM25+BERT-Large(Zero-Shot) & 0.558 & 0.399\up{11.8}\\
BM25+RM3+BERT-Large(Zero-Shot) & 0.559 & 0.395\up{10.6}\\
BM25+T5(Zero-Shot) & 0.591 & 0.408\up{14.3}\\
BM25+RM3+T5(Zero-Shot) & 0.577 & 0.396\up{10.9} \\
\midrule
\multicolumn{3}{l}{\bf CAR + Rank Fusion} \\
\bart{} (paa) & 0.533 & 0.370\up{3.53}\\
\vinci{} & 0.551 & 0.378\up{5.74}\\
\chatgpt{} & 0.555 & 0.381\up{6.81}\\


\midrule
\multicolumn{3}{l}{\bf CAR + QPP + Rank Fusion} \\

\bart{} (paa) & 0.631 & 0.3755\up{5.2}\\
\vinci{} & 0.628 & 0.3809\up{6.7}\\
\chatgpt{} & 0.637 & 0.3837\up{7.5}\\
        \bottomrule        
    \end{tabular}

    
    \caption{Results for our model: Rank Fusion of BERT and our ambiguous model}
    % \vspace{-5mm}
    \label{tab:reranking-msmarco-hard-doc}
\end{table}


==> tables/table-anecdotal.tex <==
\begin{table*}
\begin{tabular}{lp{.82\textwidth}}
\toprule
    \textbf{Method}     & \textbf{Query Text} \\
\midrule
\textbf{Original query}  & \textbf{define sri}\\
\qd{}  & SRI stands for "Stanford Research Institute," which is a nonprofit research organization that was founded in 1946 as part of Stanford University. Over the years, SRI has conducted groundbreaking research in a wide range [\dots] \\
\vinci{}  & Sri is a Sanskrit word meaning “holy” or “auspicious.” It is often used in Hinduism as an honorific title for a deity or spiritual teacher. It is also used in Buddhist and Jain contexts, and is an important concept in South Asian culture. \\
\chatgpt{}  & Find the definition and meaning of the acronym SRI (Socially Responsible Investing).\\
\car (\vinci{})  & What is the meaning of Sanskrit word "Sri" and how is it used as a title of veneration? \\
\car (\chatgpt{})  & What is the meaning of the Sanskrit word "Sri" and how is it used in Indian subcontinent?\\
% \car (\vinci{})(doc)  & What is the origin and meaning of the term "Sri"? \\
% \car (\chatgpt{})(doc)  & What is the origin of the word "Sri" used in India and other South Asian countries?\\
\midrule
\midrule

\textbf{Original query}  & \textbf{hs worms}\\
\qd{}  & HS Worms can refer to several different things depending on the context. If you are referring to HS Worms as an educational institution, then it stands for Hochschule Worms which is a university of applied sciences or it can refer to heartworms [\dots] \\
\vinci{}  & Find information about heartworms in dogs\\
\chatgpt{}  & Find information about the symptoms, causes, and treatment options for heartworm disease in dogs (also known as HS worms).\\
\car (\vinci{})  & What are the courses offered by Hochschule Worms?\\
\car (\chatgpt{})  & What are the programs offered by Hochschule Worms?\\
% \car (\vinci{})(doc)  & What is the country rank and world rank of HS Worms University?\\
% \car (\chatgpt{})(doc)  & What is Hochschule Worms (HS Worms) and where is it located?\\
\midrule
\midrule

\textbf{Original query}  & \textbf{ephesians 6:5-9}\\
\qd{}  & Ephesians 6:5-9 is a passage from the New Testament that speaks to the relationship between slaves and masters in ancient times. It begins by instructing slaves to obey their earthly masters with respect [\dots] \\
\vinci{}  & Find information about Ephesians 6:5-9.\\
\chatgpt{}  & What is the meaning and interpretation of Ephesians 6:5-9 in the Bible?\\
\car (\vinci{})  & 7 With good will render service, as to the Lord, and not to men, 8 knowing that whatever good thing each one does, this he will receive back from the Lord\\
\car (\chatgpt{})  & How does the passage in Ephesians 6:5-9 instruct slaves to behave towards their masters?\\
% \car (\vinci{})(doc)  & too have a Master in heaven. What does Ephesians 6:5-9 teach about the relationship between slaves and masters? \\
% \car (\chatgpt{})(doc)  & What is the meaning of Ephesians 6:5-9 in relation to submission and slavery?\\
\midrule
\midrule

\textbf{Original query}   & \textbf{price nrz}\\
\qd{}  & Price NRZ stands for "Non-Return-to-Zero" and refers to a digital signal encoding technique used in telecommunications. In this technique, the voltage level of the signal remains constant during each bit interval[\dots] \\
\vinci{}  & Find information on the Pricing of Non-Recourse Z-Bonds.\\
\chatgpt{}  & Find information on the pricing strategy for non-return-to-zero (NRZ) encoding.\\
\car (\vinci{})  & What is the pricing of New Residential Investment Corp. common stock on Jan 30, 2017 7:16 PM EST?\\
\car (\chatgpt{})  & What is the public offering price of New Residential Investment Corp.'s common stock?\\
% \car (\vinci{})(doc)  & announced today that it has entered into definitive agreements to acquire Shellpoint Partners, LLC ("Shellpoint"), a leading mortgage servicer and originator.hat is the price of New Residential Investment Corp (NRZ) stock \\
% \car (\chatgpt{})(doc)  & What is the current share price and financial information of New Residential Investment Corp (NRZ)?\\
\midrule

\end{tabular}
\caption{Comparing \textbf{Original} ambiguous queries with their rewrites using \qd{}, \vinci{}, \chatgpt{} approach with in-context and context aware rewriter(\car{}) techniques.}
% Approach with \textbf{(doc)} are rewrites using \ms{} document corpus and the rest from \ms{} passage corpus.
\label{tab:anecdotal_or}
\vspace{-0.25cm}
\end{table*}


==> tables/table-intro-anecdotal.tex <==
\begin{table*}[hbt!]
\begin{tabular}{lp{0.9\textwidth}}
\midrule
\textbf{Query:}  & \textbf{``anthropological definition of environment''}\\
\midrule
\textbf{BR} & Anthropology is the scientific study of human beings as social organisms interacting with each other in their environment, and cultural aspects [\dots] \\
\textbf{SR} & Environmental anthropology is a sub-specialty within the field of anthropology that takes an active role in examining the relationships between humans and their environment across space and time[\dots] \\
\midrule
\textbf{Query:}  & \textbf{``what is famvir prescribed for''}\\
\midrule
\textbf{BR} & What can be done and what is being done. First and foremost, physicians have to STOP prescribing as many drugs as they are prescribing, [\dots]\\
\textbf{SR}  & Famvir (Famciclovir) is approved by the FDA for the treatment of cold sores. If started at the first sign of symptoms, taking a single high dose [\dots]\\
\midrule
%\textbf{Query:}  & \textbf{``symptoms of different types of brain bleeds''}\\
%\midrule
%\textbf{BR} & Symptom categories related to Bleeding in the brain may include: 1 Brain symptoms (2787 causes) 2 Bleeding symptoms (1783 causes) 3 Head [\dots]\\
%\textbf{SR}  & Intracerebral hemorrhage. Intracerebral hemorrhage (ICH), also known as cerebral bleed, is a type of intracranial bleed that occurs within the brain  [\dots] \\
%\midrule
%\textbf{Query:}  & \textbf{``why does lacquered brass tarnish''}\\
%\midrule
%\textbf{BR} & How to Patina Brass. Patina is a natural tarnish that forms on the surface of brass and other metals. Adding a patina finish to brass pieces can give  [\dots](0)\\
%\textbf{SR}  & Lacquered Brass A modern take on brass is to coat it with a protective laquer coating. This may work for a while (depending on lacquered quality) but  [\dots](3) \\
%\midrule
\end{tabular}
\caption{Comparing top-1 document retrieved by Base Ranker and our Specialized Ranker for two sample hard queries.}
\label{tab:intro_anecdotal}
\vspace{-5mm}
\end{table*}


==> tables/table-ranking-combined.tex <==
\begin{table*}
    \centering
    \begin{tabular}{p{.13\textwidth}p{.13\textwidth}p{.12\textwidth}p{.12\textwidth}p{.12\textwidth}|lp{.12\textwidth}p{.12\textwidth}p{.12\textwidth}p{.12\textwidth}}
    %\begin{tabular}{lcccc|lcccc}
        \toprule
            & \multicolumn{4}{c}{\textbf{\trecdl{} Passage}} && \multicolumn{4}{c}{\textbf{\trecdl{} Document}}\\
             \midrule
            & \multicolumn{2}{c}{\textbf{\trecdl{}-19}} & \multicolumn{2}{c}{\textbf{\trecdl{}-20}} && \multicolumn{2}{c}{\textbf{\trecdl{}-19}} & \multicolumn{2}{c}{\textbf{\trecdl{}-20}}\\
            \cmidrule(lr){2-3}
            \cmidrule(lr){4-5}
            \cmidrule(lr){7-8}
            \cmidrule(lr){9-10}
            \textit{Ranking Models}
            &  $\text{RR}$ & $\text{nDCG}_\text{10}$ &  $\text{RR}$ & $\text{nDCG}_\text{10}$ &&  $\text{RR}$ & $\text{nDCG}_\text{10}$ &  $\text{RR}$ & $\text{nDCG}_\text{10}$ \\
            \midrule

%% RR and nDCG@10 scores
\multicolumn{5}{l}{\bf Baseline} \\
\bert{} Baseline &  0.653 & 0.381 &  0.523 & 0.288 && 	0.750 &	0.453 & 	0.735 &	0.393 \\	
\qd{}~\cite{wang2023query2doc} &  0.578\down{11.6}$^{\#}$ & 0.321\down{15.7} &  0.608\up{16.2} & 0.323\up{12.3} && 	\textbf{0.82\up{9.7}} &	0.467\up{3.1}$^{*}$ & 	0.749\up{2} &	0.415\up{5.6}$^{*}$ \\
\midrule
\multicolumn{5}{l}{\bf Query expansion} \\
\bart{} (topic)     &  0.500\down{23.5}$^{*}$ & 0.254\down{33.3}$^{*}$ &  0.380\down{27.3}$^{*}$ & 0.202\down{29.9}$^{*}$ && - & - & - & - \\
\ada{} &  0.634\down{2.9} & 0.370\down{2.9} &  0.479\down{8.4} & 0.278\down{3.6} && - & - & - & - \\
\babbage{} &  0.697\up{6.7} & 0.370\down{3.0} &  0.580\up{10.9} & 0.327\up{13.5} && - & - & - & - \\
\curie{} &  0.563\down{13.9} & 0.328\down{13.9} &  0.498\down{4.8} & 0.248\down{13.8} && - & - & - & - \\
\davinci{} &  0.795\up{21.7}$^{*}$ & 0.391\up{2.6} &  0.507\down{3.1} & 0.284\down{1.3} && - & - & - & - \\
 \vinci{} (prompt1) &  0.714\up{9.4} & 0.386\up{1.3} &  0.493\down{5.7} & 0.289\up{0.4} && - & - & - & - \\
\vinci{} (prompt2) &  0.717\up{9.9} & 0.397\up{4.1} &  0.574\up{9.7} & 0.338\up{17.3} && - & - & - & - \\
\vinci{}  &  0.766\up{17.3}$^{\#}$ & 0.411\up{7.9} &  0.552\up{5.6} & 0.308\up{7.1} && 	\underline{0.818\up{9.1}} &	0.490\up{8.2}$^{\#}$ & 	0.764\up{4.0} &	0.465\up{18.5}$^{\#}$ \\
\chatgpt{} &  0.689\up{5.5} & 0.396\up{4.0} &  \underline{0.623\up{19.2}}$^{\#}$ & 0.348\up{20.7}$^{\#}$ && - & - & - & - \\	
\midrule
\midrule
\multicolumn{5}{l}{\bf \car{}} \\
\bart{} (topic+PAA) &  0.745\up{14.2} & 0.391\up{2.6} &  0.614\up{17.4}$^{*}$ & \underline{0.363\up{26.0}} && 	0.762\up{1.6} &	0.504\up{11.3}$^{\#}$ & 	\underline{0.819\up{11.5}} &	\underline{0.485\up{23.4}}$^{\#}$ \\
\vinci{} & \textbf{0.798\up{22.2}}$^{*}$ & \underline{0.417\up{9.5}} &  0.533\up{2.0} & 0.316\up{9.9} &&	0.774\up{3.3} &	0.507\up{12.0}$^{*}$ & 	0.777\up{5.8} &	0.447\up{13.7}$^{*}$ \\
\chatgpt{} &  \underline{0.794\up{21.6}}$^{*}$ & \textbf{0.494\up{29.7}}$^{*}$ &  \textbf{0.653\up{24.8}}$^{*}$ & \textbf{0.383\up{33.1}}$^{*}$ && 	0.769\up{2.6} &	\underline{0.509\up{12.3}}$^{\#}$ & 	0.7826\up{6.5} &	0.430\up{9.4}$^{*}$ \\
\vinci{} (\attention{}) & - & - & - & - && 0.81\up{8.1} & \textbf{0.517\up{14.1}}$^{*}$ & 0.785\up{6.9} & 0.459\up{17}$^{\#}$ \\
\vinci{} (\linear{}) & - & - & - & - && 0.782\up{4.3} & 0.497\up{9.7}$^{*}$ & \textbf{0.848\up{15.5}} & \textbf{0.504\up{28.4}}$^{*}$ \\
\chatgpt{} (\attention{}) & - & - & - & - && 0.759\up{1.3} &	0.465\up{2.6} & 0.773\up{5.3} &	0.417\up{6.2}$^{*}$ \\
\chatgpt{} (\linear{}) & - & - & - & - && 0.778\up{3.8}	& \textbf{0.517\up{14.1}}$^{*}$ & 0.799\up{8.8} &	0.461\up{17.5}$^{*}$ \\


        \bottomrule        
    \end{tabular}

    
    \caption{Ranking performance of \bert{} model trained using query expansions from different query generative models on \trecdl{} '19 and \trecdl{} '20. We show the relative improvement of our approaches against a baseline (fine-tuned on original queries without query expansion) in parentheses. Statistically significant improvements at a level of $95\%$ and $90\%$ are indicated by $*$ and $\#$ respectively~\cite{paired_significance_test}. The best results for each dataset and each model is in \textbf{bold} and second is \underline{underlined}. \todo {Remove RR values to fit or have different tables(already present in ictir project) for passage and document collection.}}
    \vspace{-5mm}
    \label{tab:reranking-msmarco}
\end{table*}


==> tables/table-rewriter.tex <==
\begin{table}[hbt!]
\centering
\begin{tabular}{llll|r}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{BERTScore}} & \multirow{2}{*}{\textbf{Rouge-L}} \\
\cmidrule(lr){2-4}
  & \textbf{P}     & \textbf{R}     & \textbf{F1}    &  \\
\hline

GPT2 (topic){$^\dagger$}                   & 0.457          & 0.447          & 0.451          & 7.47            \\
\bart{} (topic){$^\dagger$}        & 0.792          & 0.791          & 0.792          & 28.89           \\
\qd{}  & 0.672 & 0.749 & 0.708 & 6.76 \\
\ada{}  (in-context)         & 0.734          & 0.776          & 0.754            & 17.43            \\
\babbage{} (in-context)           & 0.804          & 0.802          & 0.802          & 32.16            \\
\curie{} (in-context)          & 0.812          & 0.800          & 0.805          & 34.25            \\
\davinci{} (in-context)           & 0.818         & 0.823          & 0.820        & 33.81            \\
\vinci{} (prompt1)            & 0.727          & 0.743          & 0.734          & 14.38          \\
\vinci{} (prompt2)            & 0.811          & 0.792          & 0.801          & 32.07           \\
\vinci{} (in-context)         & 0.817 & 0.818 & 0.817 & 34.68  \\
\chatgpt{}           & 0.768          & 0.812          & 0.789          & 25.77           \\
\hline
\multicolumn{5}{l}{\bf  \car{}} \\
\bart{} (topic+PAA){$^\dagger$}  & 0.777          & 0.783          & 0.779          & 25.85           \\
\vinci{} &\underline{0.821} & \underline{0.834} & \underline{0.827} & \underline{38.57}  \\
\chatgpt{} & \textbf{0.825} &  \textbf{0.847} &  \textbf{0.836} & \textbf{40.51}\\ \hline
\end{tabular}
\caption{BERTScore and ROUGEL scores for different rewrites on TREC web 2012. The best results for each dataset and each model is in \textbf{bold} and second is \underline{underlined}. {$^\dagger$}indicates that the model has been fine-tuned with topic or topic + PAA data.}
\label{tab:rewriter}
\end{table}

==> tables/tables-gpt3.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|l|c|}
    \hline
        \textbf{Model} & \textbf{\# parameters}  \\\hline
         \texttt{text-ada-001} (\ada{}) &  350M \\
          \texttt{text-babbage-001} (\babbage{})  & 3B\\
          \texttt{text-curie-001 }(\curie{}) & 13B \\
         \texttt{text-davinci-002} (\davinci{}) & 175B \\
         \texttt{text-davinci-003 }(\vinci{})  & 175B \\
         \texttt{gpt-3.5-turbo }(\chatgpt{})  & 154B \\
          

  \hline
    \end{tabular}
    \caption{LLM (GPT3 models) of different parameter scales}
    \label{tab:gpt3_scales}
\end{table}

==> tables/wice/wice_performance.tex <==
\begin{table}[htb!]
\centering
\footnotesize
\begin{tabular}{c c c c c c c c}
\multirow{2}{*}{Experiment setting} & \multirow{2}{*}{Accuracy} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{Precision} & \multicolumn{2}{c}{Recall}  \\ 
\cline{3-8}
  & &  Weighted  & Macro & Weighted & Macro & Weighted & Macro      \\
\hline
\multicolumn{1}{l}{\textit{Sparse + Re-ranking}} & & & & \\
Full-Wiki & \textbf{63.69} &  \textbf{61.84} &  \textbf{55.24} &  \textbf{61.12} &  \textbf{56.54} &  \textbf{63.69} &  \textbf{55.32 } \\
Claim detection & 61.90 & 60.12 & \underline{53.33} & 59.27 & 54.26 & 61.90 & \underline{53.53} \\
Citation Extraction & 61.01 & 59.56 & 52.96 & 58.75 & 53.59 & 61.01 & 53.09 \\
Fusion & \underline{63.39} & \underline{60.21} & 52.48 & \underline{59.46} & \underline{54.69} & \underline{63.39} & 53.27  \\[5mm]

\hline
\multicolumn{1}{l}{\textit{Dense Retrieval}} & & & & \\
Full-Wiki &  61.61 & 60.95 & 55.21 & 60.47 & 55.49 & 61.61 & 55.13 \\
% Full-Wiki  & 60.42 & 58.80 & 51.96 & 57.90 & 52.58 & 60.42 & 52.19 \\
Claim detection & 61.01 & 58.94 & 51.78 & 57.96 & 52.70 & 61.01 & 52.17 \\
Citation Extraction & 58.63 & 58.48 & \underline{52.92} & 58.35 & 52.95 & 58.63 & \underline{52.91} \\
Fusion & \underline{61.31} & \underline{59.34} & 52.30 & 58.40 & \underline{53.23} & \underline{61.31} & 52.62  \\[5mm]

\hline
\multicolumn{1}{l}{\textit{Index Compression}} & & & & & & &  \\
Full-Wiki & 62.46 & 61.38 & 55.27 & 60.74 & 55.84 & 62.46 & 55.20  \\
% Original  & 60.46 & 60.63 & 55.64 & 60.81 & 55.60 & 60.46 & 55.70  \\
Claim detection & 59.31 & 59.02 & \underline{53.32} & 58.77 & 53.39 & 59.31 & \underline{53.30}  \\
Citation Extraction & 60.74 & 59.21 & 52.42 & 58.34 & 53.04 & 60.74 & 52.60  \\
Fusion & \underline{63.04} & \underline{59.79} & 51.89 & 58.94 & \underline{53.97} & \underline{63.04} & 52.76 \\[5mm]

\hline
\end{tabular}
\caption{Performance experiments on WiCE data and adjustments using full document text of English Wikipedia. The bold-styled values represent the baseline while the underlined-styled values represent the highest scores of the re-ranked data within a retrieval setup category.}
\label{tab:wice_performance_metrics}
\end{table}
% Full document text 
% 
